Designing a Multi-Objective Reward Function for Creating Teams of Robotic Bodyguards Using Deep Reinforcement Learning

We are considering a scenario where a team of bodyguard robots provides physical protection to a VIP in a crowded public space. We use deep reinforcement learning to learn the policy to be followed by the robots. As the robot bodyguards need to follow several difficult-to-reconcile goals, we study several primitive and composite reward functions and their impact on the overall behavior of the robotic bodyguards.

==> Approach.tex <==
\section{Approach}
\label{sec:Approach}

\subsection{Environment model}

{\color{blue}

\begin{itemize}
    \item Describe the scenario (market, VIP, bodyguards, bystanders etc)
    \item Describe the movement patterns of the VIP
    \item Describe the movement pattern of the bystanders. Describe whatever algorithms you used to stop them before bumping into things.
    \item Explain that the learning will only impact the bodyguards.
    \item Describe the software framework you have used. Relate the problem here to other problems this framework was used to model (predator-prey, etc.)
    \item Add a screenshot here explaining the environment
\end{itemize}

}

\subsection{Learning framework}

{\color{blue}
\begin{itemize}
    \item Describe how the learning is processing - reinforcement learning, how it is done, where are the rewards coming from, when is the policy updated etc.
    \item Present the RL algorithms used
    \item Discuss shared learning of multiple bodyguards
\end{itemize}
}

\subsection{Engineering the reward}

{\color{blue}
\begin{itemize}
    \item Discuss the challenges of designing an appropriate reward. There is no mathematical formulation of what a bodyguard needs to do.
    \item We start from the protection metric --- how is that incorporated into the reward? (is it a negative???)
    \item Discuss emergent phenomena - bodyguards assaulting the VIP, etc. Possibly with screenshots here.
    \item Discuss how do you fix the emergent phenomena - by adding additional criteria to the reward.
\end{itemize}
}


==> ThreatLevel.tex <==
\section{Quantifying the threat level to the VIP}
\label{sec:Threat}

The overall objective of a bodyguard is to protect a VIP from assault, harassment and other dangers. In order to measure the effectiveness of the bodyguards, we need a numerical measure of the threat faced by the VIP. To create this definition, we are going to use as starting point the definitions provided in~\cite{Bhatia-2016-FLAIRS}. We are considering a VIP who is moving in crowd of bystanders $\mathcal{B}=\left\{ b_{1},b_{2},\ldots,b_{m}\right\}$
surrounded by a group of robot bodyguards $R=\left\{ r_{1},r_{2},\ldots,r_{n}\right\}$.

Two agents $x$ and $y$ have a {\em line of sight} $LoS(x,y)\in\left[0,1\right]$ if the agent $x$ can directly observe agent $y$ and vice verse without having obstacle between them. We also introduce the notion of {\em safe distance} $SafeDist\left(VIP,b_{i}\right)$. If $Dist\left(VIP,b_{i}\right)\geq SafeDist\left(VIP,b_{i}\right)$ then the VIP is considered safe from the crowd member $b_{i}$.

The {\em threat level} $TL\left(VIP,b_{i}\right)$ is defined as the probability
that a member of the crowd $b_{i}$ can successfully assault the VIP, defined as a value exponentially decaying with distance:
\[
TL\left(VIP,b_{i}\right)=\exp^{-A\left(Dist(VIP,b_{i})\right)/B}
\]
\noindent where the VIP should be in line of sight of the crowd member $b_{i}$
and the $Dist(VIP,b_{i})<SafeDist\left(VIP,b_{i}\right)$. $A$ and
$B$ are positive constants that control the decaying rate of the
threat level.


\subsection{Total Threat}

The total threat to the VIP from crowd $\mathcal{B}$ is over the
time $T$ is defined as:
\[
TT=\intop_{0}^{T}1-\prod_{i=1}^{k}\left(1-TL\left(VIP,b_{i}\right)\right)dt
\]


The total threat to the VIP depends on the movement of the VIP and
the robot bodyguards along with its speed at which he is moving in
the crowd.

